Study of the $B_c^+$ decays into charmonia and three light hadrons

Using proton-proton collision data, corresponding to an integrated luminosity of $9fb^{-1}$ collected with the LHCb detector, seven decay modes of the $B_c^+$ meson into a $J/\psi$ or $\psi(2S)$ meson and three charged hadrons, kaons or pions, are studied. The decays $B_c^+\rightarrow ( \psi(2S) \rightarrow J/\psi \pi^+ \pi^-)\pi^+ $, $B_c^+\rightarrow \psi(2S)\pi^+\pi^+\pi^-$, $B_c^+\rightarrow J/\psi K^+\pi^+\pi^-$ and $B_c^+\rightarrow K^+K^+K^-$ are observed for the first time, and evidence for the $B_c^+\rightarrow \psi(2S)K^+K^-\pi^+$ decay is found, where $J/\psi$ and $\psi(2S)$ mesons are reconstructed in their dimuon decay modes. The ratios of branching fractions between the different $B_c^+$ decays are reported as well as the fractions of the decays proceeding via intermediate resonances. The results largely support the factorisation approach used for a theoretical description of the studied decays.

==> Authorship_LHCb-PAPER-2021-034-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abell{\'a}n Beteta,
F.J. Abudinen Gallego,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista Leite,
M. Barbetti,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
S. Bashir,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
S. Bifani,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
I. Corredoira ,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Dashkina,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. F{\'e}o,
A. Fernandez Prieto,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
A. Fkiaras,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
E. Gabriel,
G. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
M. Guittiere,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
T. Halewood-leagas,
P.M. Hamilton,
J.P. Hammerich,
Q. Han,
X. Han,
T.H. Hancock,
E.B. Hansen,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
X. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S.H. Kalavan Kadavath,
S. Kandybei,
Y. Kang,
M. Karacson,
M. Karpov,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P. Li,
S. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
S. Lopez Solino,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Madejczyk,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
N.T. Mchugh,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
D.P. O'Hanlon,
S. Okamura,
R. Oldeman,
F. Oliva,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
M. Pizzichemi,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
H. Pullen,
G. Punzi,
H. Qi,
W. Qian,
J. Qin,
N. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
E.R.R. Rodriguez Rodriguez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
K.A. Thomson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
X. Tong,
D. Torres Machado,
D.Y. Tou,
E. Trifonova,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
S.G. Weber,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
J.B. Zonneveld,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica
